Visual Designs for Binned Aggregation of Multi-Class Scatterplots

Point sets in 2D with multiple classes are a common type of data. A canonical visualization design for them are scatterplots, which do not scale to large collections of points. For these larger data sets, binned aggregation (or binning) is often used to summarize the data, with many possible design alternatives for creating effective visual representations of these summaries. There are a wide range of designs to show summaries of 2D multi-class point data, each capable of supporting different analysis tasks. In this paper, we explore the space of visual designs for such data, and provide design guidelines for different analysis scenarios. To support these guidelines, we compile a set of abstract tasks and ground them in concrete examples using multiple sample datasets. We then assess designs, and survey a range of design decisions, considering their appropriateness to the tasks. In addition, we provide a web-based implementation to experiment with design choices, supporting the validation of designs based on task needs.

==> figures.tex <==
\newcommand\designChoice{
	\begin{figure}
		\centering
		\includegraphics[width=\columnwidth]{images/design_choice.pdf}
		\caption{
			Design space for binned scatterplots.
			The first three categories are relevant for the representation of bins, while the last three categories deal with the representation of classes and class distributions.
		}
		\label{designChoice}
	\end{figure}
}

\newcommand\nbabinall{
	\begin{figure*}[t!]
		\centering
		\includegraphics[width=\textwidth]{images/nba_all.pdf}
		\caption{Shooting positions for four \emph{guards}, 1~\crule[p1]{0.25cm}{0.25cm},
			2~\crule[p2]{0.25cm}{0.25cm}, 
			3~\crule[p3]{0.25cm}{0.25cm}, and
			4~\crule[p4]{0.25cm}{0.25cm},
			from the NBA dataset.
			(a) only conveys rough densities.
			(b) is a design of binned aggregation that uses a grayscale color map in the background to show the total number of data points in each bin.
			In addition, each bin includes a pie chart that shows class proportions in that bin.
			(c) is a juxtaposition-based design of binned aggregation.
			Each class is shown in a separate plot.
			Binned aggregation lets users discern much more information from the data than the tradition scatterplot that has overplotting issues.}
		\label{nbabinall}
	\end{figure*}
}

\newcommand\treecoverall{
	\begin{figure*}[t!]
		\centering
		\includegraphics[width=\textwidth]{images/trees_all.pdf}
		\caption{
			These plots are based on the Tree Cover in Colorado dataset.
			It has seven different tree types: \crule[spruce]{0.25cm}{0.25cm} spruce and fir,
			\crule[lodgepole]{0.25cm}{0.25cm} lodgepole pine,
			\crule[ponderosa]{0.25cm}{0.25cm} ponderosa pine,
			\crule[cottonwood]{0.25cm}{0.25cm} cottonwood / willow,
			\crule[aspen]{0.25cm}{0.25cm} aspen,
			\crule[douglas]{0.25cm}{0.25cm} douglas fir, and
			\crule[krumm]{0.25cm}{0.25cm} krummholz.
			In the scatterplot (a), details about the distribution of classes are hard to discern due to overplotting.
			The second visualization (b) is created using binned aggregation.
			It allows to compare bin density encoded by the pie sizes.
			In addition, class diversity is also shown by the pie charts.
			The third visualization (c) shows class identity within each bin and provides better information about minority classes.
			The fourth visualization (d) shows distributions for two classes (\crule[lodgepole]{0.25cm}{0.25cm} and \crule[spruce]{0.25cm}{0.25cm}) based on a bar chart design.
			It allows us to compare their respective distributions.
		}
		\label{treecoverall}
	\end{figure*}
}

\newcommand\ldaall{
	\begin{figure*}[t!]
		\centering
		\includegraphics[width=1.0\textwidth]{images/lda_combined.pdf}
		\caption{
			These plots are based on the Early Modern Drama corpus.
			It comprises nine types of dramatic texts:
			\crule[tr]{0.25cm}{0.25cm} tragedy,
			\crule[tc]{0.25cm}{0.25cm} tragicomedy,
			\crule[co]{0.25cm}{0.25cm} comedy,
			\crule[hi]{0.25cm}{0.25cm} history,
			\crule[ma]{0.25cm}{0.25cm} masque,
			\crule[in]{0.25cm}{0.25cm} interlude,
			\crule[en]{0.25cm}{0.25cm} entertainment,
			\crule[di]{0.25cm}{0.25cm} dialogue, and
			\crule[nd]{0.25cm}{0.25cm} non-dramatic.
			In the scatterplot (a), details about the distribution of classes and overlap are hard discern due to overplotting.
			The second plot (b) shows rough densities of the entire dataset based on color weaving.
			The third visualization (c) shows rectangular bins of the data, color based on high class-internal frequency values that convey a sense of regions with density peaks for each class.
			(d) is a small multiple design per bin that encodes frequencies for each class showing regions of overlap and extensions of classes.
		}
		\label{ldaall}
	\end{figure*}
}

\newcommand\blendWeaveAndHatch{
	\begin{figure*}
		\centering
		\includegraphics[width=\textwidth]{images/blend_weave_and_hatch.pdf}
		\caption{
			Three visualizations of an artificially generated dataset with four different classes (\classred, \classgreen, \classblue, \classorange).
			(a) demonstrates color blending, which uses binned color and saturation to encode class labels and their intensity.
			(b) demonstrates weaving with bin-internal normalization, resulting in fully filled bins with the number of colored fragments encoding bin-relative class intensities.
			(c) demonstrates hatching, which uses both angle and color to encode class labels.
		}
		\label{fig:blend_weave_and_hatch}
	\end{figure*}
}

\newcommand\designTaskGrid{
	\begin{table}[t!]
		\centering
		\includegraphics[width=\columnwidth]{images/discussion_table.pdf}
		\caption{
			This table summarizes the discussion of Section~\ref{sec:design} by mapping design aspects to tasks.
			A check mark means a design is appropriate for the task; a circle means the design supports (aspects of) the task but may not be the best choice for it; an X means the design does not support the task.
			% This table helps finding combinations of designs combining suitable (see Section~\ref{sec:design}) design aspects of which the combined task row contains check marks for the tasks to support.
		}
		\label{table:designTasks}
		\vspace{-6mm}
	\end{table}
}

\renewcommand*{\arraystretch}{1.3}
\newcolumntype{K}{p{0.3cm}}
\newcolumntype{N}{>{\raggedright\arraybackslash}p{6cm}}
\newcommand\newTasksTable{
	\begin{table*}
		\begin{center}
			\begin{tabular}{@{}Klr@{\hskip4pt}Nr@{\hskip4pt}N@{}} \toprule
			 & Task	& \multicolumn{2}{l}{Bin-centric} & \multicolumn{2}{l}{Class-centric} \\ \midrule
			 & Explore neighborhood & 1 & Explore properties of bins in a neighborhood & 2 & Explore properties of classes in a neighborhood \\
			 & Search for known motif & 3 & Find known pattern across bins & 4 & Find known pattern across classes \\ 
			\multirow{-3}{*}{\adjustbox{margin=0 0 2.4mm 0,set height=0.3cm,angle=90}{browsing}} & Explore data & 5 & Unusual patterns within or across bins, global trends between bins & 6 & Unusual patterns within or across classes, global trends within or between classes \\ \midrule
			 & Characterize distribution & 7 & Do bins close to each other have similar properties? Or within a certain area or range of values? & 8 & Does a class occupy certain areas of the plot? Does its distribution have a particular shape? Do classes correlate in certain areas? \\
			 & Identify anomalies & 9 & Identify bins that are outliers based on the general distribution & 10 & Identify classes or subsets of classes that are outliers in a certain region \\
			 & Identify correlation & 11 & Determine level of correlation of bin properties along both dimensions & 12 & Determine level of correlation for class members along both dimensions \\
			 & Numerosity comparison & 13 & Compare density in different regions of the space & 14 & Compare class density in different regions of the space \\
			\multirow{-8}{*}{\adjustbox{margin=0 0 1mm 0,set height=0.3cm,angle=90}{aggregate-level}} & Understand distances & 15 & Understand a given spatialization and the coverage of the bins & 16 & Understand a given spatialization and the coverage of classes \\
			\bottomrule
			\end{tabular}
		\end{center}
		\caption{
			Tasks for binned scatterplots, based on the general scatterplot tasks compiled and categorized by Sarikaya and Gleicher~\cite{Sarikaya2018}.
			We reduced the original, larger set of tasks to those that capture high-level data characteristics according to the definition by Schulz~\etal~\cite{Schulz2013}.
			For binned scatterplots, each of the resulting tasks can have a \emph{bin-centric} or a \emph{class-centric} scope.
		}
		\label{targetTable}
		\vspace{-6mm}
	\end{table*}
}


==> tex/case.tex <==
We have collected several 2D datasets from different domains with multiple classes.
In this section, we showcase three different example analyses based on each of them.
We have picked these use cases to serve as a motivation for why binned aggregation methods are important.
In addition, we will derive multiple representative tasks from them on which we will base the discussion of our design space.
%All of these datasets have 4 to 7 different classes.
Each of the datasets has a large number of items and exhibits overplotting problems at usual display resolutions.
%We chose datasets from different domains to show the generality of this problem.
%We include some possible questions that will be asked for each dataset.
%We then discuss how binned aggregation would better help answer these questions. 

\subsection{Fatality Analysis Reporting System (FARS) Dataset} 
This is a dataset about fatal car crashes that includes car crashes in California from 2011-2015 \cite{farsdata2017}. We picked 5 of the most common crash types in the dataset and investigate their distribution. Figure \ref{farsall}(a) shows a scatterplot based on this dataset. We can see rough distribution that car crashes happen more in big cities. Figure \ref{farsall}(b) shows a splatterplot \cite{Mayorga2013} version of this dataset. Splatterplot is a design of KDE that shows aggregated information. We have clearer overview of the most dense area in this figure and relative density of a specific class. However, both scatterplot and splatterplot do not clearly show which crash type happens more often. Figure \ref{farsall}(c) shows a design of binned aggregation. In this figure, we can see that car crashes happen more in big cities and south California has more accidents. It is not surprising to see this since the traffic is heavier in cities. Los Angelas is a ``cars first" city, so it is reasonable to see more car crashes in Los Angelas. By using binned aggregation, we have the freedom of focusing on specific regions (e.g., comparing San Francisco and Los Angelas) by parametrizing the size and the position of the bins.
Besides, we can see that ``Drive off Road" (labeled as 2 in Figure \ref{farsall}) is the most common crash type no matter in big cities or not from Figure \ref{farsall}(c). In that case, we might want to investigate the reason why people are more likely to drive off road. Moreover, it seems that ``Control/Traction Loss" (labeled as 1 in Figure \ref{farsall}) happens more in the south-east part of California. A possible reason might be people tend to drive faster in that region. 

\farsall
%This is a dataset about fatal car crash \cite{farsdata}. We picked three years, 2005, 2008 and 2010 from this dataset. Each year is labeled as a class and with a different color. We plotted the position of fatal car crashes in scatterplot on maps. The result is shown in Figure \ref{fars}. We can see general trend that east part of the United States has more car crash accidents. However, it is too dense in the right part that we might not be able to see whether large cities have more car accidents. It is also hard to see whether car accidents increase over these three years. In this figure, we would be interested in the questions such as: ``Which year has more car crash in Wisconsin?", ``In 2008, which area has the most number of car crashes?", ``Are there clusters of fatal car accidents in these three years?".
%\fars \farsSp \farsB
%This is from Splatterplot paper


% idea From Kwan-liu Ma paper

\subsection{Tree Cover Type Datasets} This is a standard dataset from the UCI machine learning repository \cite{Lichman2013}. It is derived from a cartographic survey of the Roosevelt National Forest of Colorado. It contains seven different kinds of tree cover types. We extracted two attributes from the dataset: elevation and horizontal distance to hydrology (nearest surface water). Elevation is the attribute that separates different tree types most. Its scatterplot is shown in Figure \ref{treecoverall}(a). Although we can see rough boundary of some classes in this figure, it is hard to see all 7 classes. It is even harder to tell proportion of different tree types in a specific region. Figure \ref{treecoverall}(b) shows the splatterplot of the dataset. In splatterplot, we can better see the range of different tree types when looking at elevation. We can also see that trees with larger elevation tend to spread out more in the domain of horizontal distance to hydrology. However, it is hard to read the color of overlapping part and we might need to carefully trace the boundary to understand the class labels. Figure \ref{treecoverall}(c) shows the dataset in binned aggregation. From this figure, we can see that the most dense part is when elevation is between 2800 - 3200 meters. Suprisingly, it is not the same area with most tree type diversity that we can clearly see in Figure \ref{treecoverall}(b). It is due to different parameters set in the function when generating splatterplot. People might have difficulty set a suitable threshold in splatterplot without enough statistic background. Yet, binned aggregation does not require this knowledge. It could show variety of tree types in a region and distribution of different tree types. It has lower chance to mislead people without concrete statistics background. From binned aggregation, we can find out that in the area with the most variety, tree type 2 has the largest proportion. We could further investigate whether tree type 2 is suitable to survive in more kinds of environments.
We can also see that tree type 1 and tree type 2 live in similar elevation and distance of hydrology. Having this information, we can further investigate whether these two tree types are competitor or mutually beneficial.

%\treecover \treecovSplatter %\treecoversp
\treecoverall

%\paragraph{Digital Humanities Datasets} \cc{More coming...}
%Splatterplot paper

%\paragraph{The Mobile User Profile Dataset}\cc{More coming...}
% Kwan-liu Ma paper

%\paragraph{Early Modern English Books Dataset} This dataset are attributes about all early modern English books transcribed by Text Creation Partnership \cite{tcp}. Figure \ref{lda} is a scatterplot plotted based on this dataset. We can see that the plot is too dense and is overplotted. It is hard to see relative density from this figure. Therefore, it needs some other type of visualization to avoid overplotting problem.

%Possible questions that people would be interested in are: ``Which type of books is more likely to use \textit{the}?", ``Do books with more \textit{the} have more \textit{and}?", ``How different (disjoint) are \textit{Play} and \textit{Science}?", ``Is there any book looking different from other books with similar usage of \textit{the} and \textit{and}?". 
%\cc{Need to revise this part to show the real label of the axis}
%\lda
